Are we pretraining it right? Digging deeper into visio-linguistic pretraining

Numerous recent works have proposed pretraining generic visio-linguistic representations and then finetuning them for downstream vision and language tasks. While architecture and objective function design choices have received attention, the choice of pretraining datasets has received little attention. In this work, we question some of the default choices made in literature. For instance, we systematically study how varying similarity between the pretraining dataset domain (textual and visual) and the downstream domain affects performance. Surprisingly, we show that automatically generated data in a domain closer to the downstream task (e.g., VQA v2) is a better choice for pretraining than "natural" data but of a slightly different domain (e.g., Conceptual Captions). On the other hand, some seemingly reasonable choices of pretraining datasets were found to be entirely ineffective for some downstream tasks. This suggests that despite the numerous recent efforts, vision & language pretraining does not quite work "out of the box" yet. Overall, as a by-product of our study, we find that simple design choices in pretraining can help us achieve close to state-of-art results on downstream tasks without any architectural changes.

==> sections/approach.tex <==
\section{Methodology}

We conduct a thorough study of different aspects of self-supervised training for vision and language. In this section we lay out our detailed methodology of analysis and how we use the insights gathered to reach near SOTA models with much less pretraining data.



\subsection{Notations}
Let us denote $\mathcal{D}^{(i)}$ as \textit{in-domain} data distribution and $\mathcal{D}^{(o)}$ as \textit{out-of-domain} data distribution. Let $\Theta_r$, $\Theta_p$ and $\Theta_f$ be the parameters of BERT initialized, pretrained and finetuned models respectively.

\subsection{Importance of self-supervised pretraining}
In the next section we show whether SSL pretraining is always beneficial before for a target downstream task in V\&L. We compare two settings : 1) Train without self-supervised pretraining stage 2) Finetune after self-supervised pretrained stage. Downstream tasks that have very different domain compared to pretraining dataset it is not always beneficial. Pretrained model deviates so much from downstream task distribution that it becomes difficult for the finetuning stage to recover it.


\subsection{Domain adaptation}
The objective of self-supervised pretraining is to learn general representations that can be transferred to the downstream task. We take two approaches of finetuning on a downstream task 

\begin{itemize}
    \item Finetune base : Finetuning the base updates parameters in the whole model. We study the effects of finetuning on a downstream task
    \item Freeze base : We freeze the base and study the generalized representations that the model learns from the pretrained task. We measure how much of these representations can be directly transfered to a downstream task. 
\end{itemize}

In both the approaches the closer the upstream dataset's domain is to that of the downstream dataset, the better accuracy is achieved. 


\subsection{Reducing the gap with out-of-domain datasets}

Current methods in V\&L pretraining require annotated data. This is a limitation as this hinders the push for truly large scale SSL for V\&L. We hypothsize that generated in-domain data with distribution $\mathcal{D}^{(g)}$ that is close to $\mathcal{D}^{(i)}$  serves as a better pretraining dataset than $\mathcal{D}^{(g)}$. With empirical results we show that downstream performance improves when the following order of pretraining data distribution is used 

\begin{equation}
   \mathcal{D}^{(i)} \gg  \mathcal{D}^{(g)} > \mathcal{D}^{(o)} 
\end{equation}

To generate \textit{in-domain} data we use a captioning model trained on in-domain data to generate captions for a large amount of images. This is then used for pretraining. 















